Can a Suit of Armor Conduct Electricity? A New Dataset for Open Book Question Answering

We present a new kind of question answering dataset, OpenBookQA, modeled after open book exams for assessing human understanding of a subject. The open book that comes with our questions is a set of 1329 elementary level science facts. Roughly 6000 questions probe an understanding of these facts and their application to novel situations. This requires combining an open book fact (e.g., metals conduct electricity) with broad common knowledge (e.g., a suit of armor is made of metal) obtained from other sources. While existing QA datasets over documents or knowledge bases, being generally self-contained, focus on linguistic understanding, OpenBookQA probes a deeper understanding of both the topic---in the context of common knowledge---and the language it is expressed in. Human performance on OpenBookQA is close to 92%, but many state-of-the-art pre-trained QA methods perform surprisingly poorly, worse than several simple neural baselines we develop. Our oracle experiments designed to circumvent the knowledge retrieval bottleneck demonstrate the value of both the open book and additional facts. We leave it as a challenge to solve the retrieval problem in this multi-hop setting and to close the large gap to human performance.

==> knowledge-model-long.tex <==
\paragraph{Knowledge-Ehnanced Reader.}
As a base knowledge-aware model we use a version of \cite{Mihaylov2018EnhanceCS}. For each instance the model reads the question $q$ and answers $c_{1..4}$ independently and attends to the set of retrieved external knowledge facts $\mathrm{K}_{Q, C}$
%$k_{1..N_{k}}$ 
to retrieve additional information. 
We do that by extending the \textbf{BiLSTM Max-Out (c)}. 
We encode each fact $k_j$ from $\mathrm{K}_{Q, C} = k_{1..N_{k}}$ ($N_{k}$ is the number of facts) with same $\BiLSTM$ context encoder as used for $q$ and $c_{1..4}$ and retrieve a single vector $r^{ctx}_{k_j} \in \mathrm{R^{2h}}$ using Eq. \ref{eq:max-h}. 
Having such representations for each $k_j$ results in knowledge memory matrix $M_k=r^{ctx}_{k_{1..N_{k}}} \in \mathrm{R^{N{k} \times 2h}}$.
Note that $M_k$ is dynamic memory, specific for each instance in the batch and is encoded on each step during training.
Each context ($ctx$) representation $r^{ctx}_{s}$ ($s \in \{q,c_1,c_2,c_3,c_4\}$) is combined with retrieved relevant knowledge $r^{kn}_s$ to obtain a knowledge-enhanced representation $r^{ctx+kn}_{s}$:
\begin{align*}
r^{kn}_{s} = sum(({M^T_k}r^{ctx}_{s}).{M_k}) \in \mathrm{R^{2h}}\\
r^{ctx+kn}_{s} = \frac{r^{ctx}_{s} + r^{kn}_{s}}{2}  \in \mathrm{R^{2h}}
\end{align*}
We then model the knowledge-enhanced attention $\alpha^{kn}_{q,c_i}$ between $q$ and $c_i$ as a linear combination of the $ctx$, $kn$ and $ctx+kn$ representations as
\begin{align*}
\alpha_{q,c_i} = W^T[Att(r^{ctx}_{s}, r^{ctx}_{c_i});Att(r^{kn}_{s}, r^{kn}_{c_i});\\
Att(r^{ctx+kn}_{s}, r^{ctx}_{c_i});Att(r^{ctx}_{s}, r^{ctx+kn}_{c_i});\\
Att(r^{ctx}_{s}, r^{kn}_{c_i});Att(r^{kn}_{s}, r^{ctx}_{c_i});\\
Att(r^{ctx+kn}_{s}, r^{kn}_{c_i});Att(r^{kn}_{s}, r^{ctx+kn}_{c_i});\\
Att(r^{ctx+kn}_{s}, r^{ctx+kn}_{c_i})]
\end{align*},
where $W \in \mathrm{R^{9}}$ is a weight vector initialized with $ones$ vector and optimized during training.
We then select the answer $c_i$ with the highest such score.
 

==> related-work-long.tex <==
\section{Related Work}
\label{sec:related}

\begin{table*}
\centering
\setlength\doublerulesep{\arrayrulewidth}
\setlength\tabcolsep{3ex}
\begin{tabular}{lllll}
\hline
Name         & Type             & Multiple & \multicolumn{2}{c}{\underline{Background Knowledge}} \\
             &                  & Hops     & Required  & Provided \\
\hline \hline
MCScript     & RC               & Some & Yes & Some \\
MultiRC      & RC               & Yes & No  & -- \\
ARC          & No context       & Some & Yes & Some \\
ProPara      & RC               & Yes/No & Yes & No \\
QAngaroo     & RC               & Yes? & No  & Yes? \\
NarrativeQA  & RC, long context & Yes & No  & -- \\
\hline
\obqa      & Partial context  & Yes & Yes & Some \\
\hline
\end{tabular}
\caption{\label{table:dataset-comparison} Comparison of \obqa with other QA datasets. RC refers to reading comprehension.}
\end{table*}


\obqa has been created so that it requires the correct answer of a question can be inferred if a science fact is combined with broadly known. Thus, we argue that in order to answer the questions human needs some base science facts (background knowledge) knowledge, broader understanding about the world (common or commonsense knowledge) and reasoning.

Initially \citet{Richardson2013-mctest-dataset}  proposed the \textit{MCTEst} dataset as a benchmark for the ability of model to reason across document context, (reading comprehension (RC)) where all the required knowledge to answer a question is contained in a document. 
It was followed by bigger datasets that framed the problem as cloze-style reading comprehension task \cite{Richardson2013-mctest-dataset,Hermann2015-rc-cnn-dm,Onishi2016-rc-whodidwhat,Hill2016-booktest}. Recently, SQuAD \cite{Rajpurkar2016-squad}, NewsQA \cite{Trischler2017-rc-newsqa} and TriviaQA \cite{joshi-EtAl:2017:Trivia-qa} proposed large scale crowd-sourced and curated datasets. 
However analysis of the datasets (cite Chen et al) and a simple features (Wiesserborn) has shown that most of the questions can be solved with context token matching (DRQA, Wieessborn) or paraphrasing which is easily exploited by the proposed models.
In the last couple of months several datasets have been created that try to propose a more challenging RC question that requires multi-step reasoning.

\paragraph{QAngaroo}\citep{QAngaroo:Welbl2017ConstructingDF} has used process of bootstrapping questions and supporting sentences (documents) by traversing a graph of connected nodes and concepts in documents from Wikipedia and medical domain. The generated questions and documents were then curated by crowd-workers to ensure unambiguity and correctness.

\paragraph{NarrativeQA} \citep{NarrativeQADeepMind2017} is a reading comprehension dataset that has been shown to require an iterative reasoning about the narrative of a story. Similar to \obqa, the questions were generated to ensure that the answer is not a direct match or paraphrase that can be retrieved with an IR approach.

\paragraph{MultiRC}\citep{MultiRCKhashabi2018} is a recent multi-choice reading comprehension dataset that is designed to require multi sentence reasoning in order to select more than one choices as answer. 

While many of the RC datasets would benefit from commonsense or background knowledge, they are designed to be solvable by the document context alone. In addition to that evaluation setup, other datasets propose using document context and external commonsense knowledge:
\paragraph{Stoy Cloze Test} \cite{Mostafazadeh2016AStories} proposed a task that requires knowledge about common everyday events in addition to the given document context in order to select a plausible ending. 
\paragraph{MCScript} is a reading comprehension dataset where,  similar \textit{Stoy Cloze Test}, the stories are designed to require everyday script knowledge. The version of the dataset was presented as a task of  \textit{SemEval-2018} where systems achieved very high results.\footnote{SemEval-2018 Task 11: Machine Comprehension using Commonsense Knowledge https://competitions.codalab.org/competitions/17184}
\paragraph{ProPara} \citep{Propara:Mishra2018TrackingSC} is a dataset that requires tracking and reasoning about the states of a process, based on its description (paragraph) and general knowledge about it, in order to answer questions.

\paragraph{ARC} \citep{ARCClark2018} is a challenging dataset for science question answering. It has two sub-subtasks. The \textit{Easy} task contains questions, mostly answerable using IR over a big text corpus. The \textit{Hard} task, that contains very hard questions, requiring deep understanding of the \textit{world} of the question and multiple reasoning steps. 
In contrast, we propose a set of science questions, that require combining




